Formal Language Constraints for Markov Decision Processes

In order to satisfy safety conditions, an agent may be constrained from acting freely. A safe controller can be designed a priori if an environment is well understood, but not when learning is employed. In particular, reinforcement learned (RL) controllers require exploration, which can be hazardous in safety critical situations. We study the benefits of giving structure to the constraints of a constrained Markov decision process by specifying them in formal languages as a step towards using safety methods from software engineering and controller synthesis. We instantiate these constraints as finite automata to efficiently recognise constraint violations. Constraint states are then used to augment the underlying MDP state and to learn a dense cost function, easing the problem of quickly learning joint MDP/constraint dynamics. We empirically evaluate the effect of these methods on training a variety of RL algorithms over several constraints specified in Safety Gym, MuJoCo, and Atari environments.

==> seaquest_2d_regex-orig.tex <==
The no-2d-dithering constraint used with the Seaquest environment was generated by a simple Python script which generated all sequences of up to 4 moves and filtered them to those which end where they begin with no side effects (e.g., pressing the fire button).

\seqsplit{((2|A)(2|A)(5|D)(5|D))|((2|A)(5|D)(2|A)(5|D))|((2|A)(5|D)(5|D)(2|A))|((5|D)(2|A)(2|A)(5|D))|((5|D)(2|A)(5|D)(2|A))|((5|D)(5|D)(2|A)(2|A))|((2|A)(2|A)(8|G)(9|H))|((2|A)(2|A)(9|H)(8|G))|((2|A)(8|G)(2|A)(9|H))|((2|A)(8|G)(9|H)(2|A))|((2|A)(9|H)(2|A)(8|G))|((2|A)(9|H)(8|G)(2|A))|((8|G)(2|A)(2|A)(9|H))|((8|G)(2|A)(9|H)(2|A))|((8|G)(9|H)(2|A)(2|A))|((9|H)(2|A)(2|A)(8|G))|((9|H)(2|A)(8|G)(2|A))|((9|H)(8|G)(2|A)(2|A))|((2|A)(3|B)(4|C)(5|D))|((2|A)(3|B)(5|D)(4|C))|((2|A)(4|C)(3|B)(5|D))|((2|A)(4|C)(5|D)(3|B))|((2|A)(5|D)(3|B)(4|C))|((2|A)(5|D)(4|C)(3|B))|((3|B)(2|A)(4|C)(5|D))|((3|B)(2|A)(5|D)(4|C))|((3|B)(4|C)(2|A)(5|D))|((3|B)(4|C)(5|D)(2|A))|((3|B)(5|D)(2|A)(4|C))|((3|B)(5|D)(4|C)(2|A))|((4|C)(2|A)(3|B)(5|D))|((4|C)(2|A)(5|D)(3|B))|((4|C)(3|B)(2|A)(5|D))|((4|C)(3|B)(5|D)(2|A))|((4|C)(5|D)(2|A)(3|B))|((4|C)(5|D)(3|B)(2|A))|((5|D)(2|A)(3|B)(4|C))|((5|D)(2|A)(4|C)(3|B))|((5|D)(3|B)(2|A)(4|C))|((5|D)(3|B)(4|C)(2|A))|((5|D)(4|C)(2|A)(3|B))|((5|D)(4|C)(3|B)(2|A))|((2|A)(3|B)(9|H))|((2|A)(3|B)(9|H))|((2|A)(9|H)(3|B))|((2|A)(9|H)(3|B))|((2|A)(3|B)(9|H))|((2|A)(9|H)(3|B))|((3|B)(2|A)(9|H))|((3|B)(2|A)(9|H))|((3|B)(9|H)(2|A))|((3|B)(9|H)(2|A))|((3|B)(2|A)(9|H))|((3|B)(9|H)(2|A))|((9|H)(2|A)(3|B))|((9|H)(2|A)(3|B))|((9|H)(3|B)(2|A))|((9|H)(3|B)(2|A))|((9|H)(2|A)(3|B))|((9|H)(3|B)(2|A))|((2|A)(3|B)(9|H))|((2|A)(9|H)(3|B))|((3|B)(2|A)(9|H))|((3|B)(9|H)(2|A))|((9|H)(2|A)(3|B))|((9|H)(3|B)(2|A))|((2|A)(4|C)(8|G))|((2|A)(4|C)(8|G))|((2|A)(8|G)(4|C))|((2|A)(8|G)(4|C))|((2|A)(4|C)(8|G))|((2|A)(8|G)(4|C))|((4|C)(2|A)(8|G))|((4|C)(2|A)(8|G))|((4|C)(8|G)(2|A))|((4|C)(8|G)(2|A))|((4|C)(2|A)(8|G))|((4|C)(8|G)(2|A))|((8|G)(2|A)(4|C))|((8|G)(2|A)(4|C))|((8|G)(4|C)(2|A))|((8|G)(4|C)(2|A))|((8|G)(2|A)(4|C))|((8|G)(4|C)(2|A))|((2|A)(4|C)(8|G))|((2|A)(8|G)(4|C))|((4|C)(2|A)(8|G))|((4|C)(8|G)(2|A))|((8|G)(2|A)(4|C))|((8|G)(4|C)(2|A))|((2|A)(5|D)(6|E)(9|H))|((2|A)(5|D)(9|H)(6|E))|((2|A)(6|E)(5|D)(9|H))|((2|A)(6|E)(9|H)(5|D))|((2|A)(9|H)(5|D)(6|E))|((2|A)(9|H)(6|E)(5|D))|((5|D)(2|A)(6|E)(9|H))|((5|D)(2|A)(9|H)(6|E))|((5|D)(6|E)(2|A)(9|H))|((5|D)(6|E)(9|H)(2|A))|((5|D)(9|H)(2|A)(6|E))|((5|D)(9|H)(6|E)(2|A))|((6|E)(2|A)(5|D)(9|H))|((6|E)(2|A)(9|H)(5|D))|((6|E)(5|D)(2|A)(9|H))|((6|E)(5|D)(9|H)(2|A))|((6|E)(9|H)(2|A)(5|D))|((6|E)(9|H)(5|D)(2|A))|((9|H)(2|A)(5|D)(6|E))|((9|H)(2|A)(6|E)(5|D))|((9|H)(5|D)(2|A)(6|E))|((9|H)(5|D)(6|E)(2|A))|((9|H)(6|E)(2|A)(5|D))|((9|H)(6|E)(5|D)(2|A))|((2|A)(5|D)(7|F)(8|G))|((2|A)(5|D)(8|G)(7|F))|((2|A)(7|F)(5|D)(8|G))|((2|A)(7|F)(8|G)(5|D))|((2|A)(8|G)(5|D)(7|F))|((2|A)(8|G)(7|F)(5|D))|((5|D)(2|A)(7|F)(8|G))|((5|D)(2|A)(8|G)(7|F))|((5|D)(7|F)(2|A)(8|G))|((5|D)(7|F)(8|G)(2|A))|((5|D)(8|G)(2|A)(7|F))|((5|D)(8|G)(7|F)(2|A))|((7|F)(2|A)(5|D)(8|G))|((7|F)(2|A)(8|G)(5|D))|((7|F)(5|D)(2|A)(8|G))|((7|F)(5|D)(8|G)(2|A))|((7|F)(8|G)(2|A)(5|D))|((7|F)(8|G)(5|D)(2|A))|((8|G)(2|A)(5|D)(7|F))|((8|G)(2|A)(7|F)(5|D))|((8|G)(5|D)(2|A)(7|F))|((8|G)(5|D)(7|F)(2|A))|((8|G)(7|F)(2|A)(5|D))|((8|G)(7|F)(5|D)(2|A))|((2|A)(5|D))|((2|A)(5|D))|((2|A)(5|D))|((5|D)(2|A))|((5|D)(2|A))|((5|D)(2|A))|((2|A)(5|D))|((2|A)(5|D))|((5|D)(2|A))|((5|D)(2|A))|((2|A)(5|D))|((5|D)(2|A))|((3|B)(3|B)(4|C)(4|C))|((3|B)(4|C)(3|B)(4|C))|((3|B)(4|C)(4|C)(3|B))|((4|C)(3|B)(3|B)(4|C))|((4|C)(3|B)(4|C)(3|B))|((4|C)(4|C)(3|B)(3|B))|((3|B)(3|B)(7|F)(9|H))|((3|B)(3|B)(9|H)(7|F))|((3|B)(7|F)(3|B)(9|H))|((3|B)(7|F)(9|H)(3|B))|((3|B)(9|H)(3|B)(7|F))|((3|B)(9|H)(7|F)(3|B))|((7|F)(3|B)(3|B)(9|H))|((7|F)(3|B)(9|H)(3|B))|((7|F)(9|H)(3|B)(3|B))|((9|H)(3|B)(3|B)(7|F))|((9|H)(3|B)(7|F)(3|B))|((9|H)(7|F)(3|B)(3|B))|((3|B)(4|C)(6|E)(9|H))|((3|B)(4|C)(9|H)(6|E))|((3|B)(6|E)(4|C)(9|H))|((3|B)(6|E)(9|H)(4|C))|((3|B)(9|H)(4|C)(6|E))|((3|B)(9|H)(6|E)(4|C))|((4|C)(3|B)(6|E)(9|H))|((4|C)(3|B)(9|H)(6|E))|((4|C)(6|E)(3|B)(9|H))|((4|C)(6|E)(9|H)(3|B))|((4|C)(9|H)(3|B)(6|E))|((4|C)(9|H)(6|E)(3|B))|((6|E)(3|B)(4|C)(9|H))|((6|E)(3|B)(9|H)(4|C))|((6|E)(4|C)(3|B)(9|H))|((6|E)(4|C)(9|H)(3|B))|((6|E)(9|H)(3|B)(4|C))|((6|E)(9|H)(4|C)(3|B))|((9|H)(3|B)(4|C)(6|E))|((9|H)(3|B)(6|E)(4|C))|((9|H)(4|C)(3|B)(6|E))|((9|H)(4|C)(6|E)(3|B))|((9|H)(6|E)(3|B)(4|C))|((9|H)(6|E)(4|C)(3|B))|((3|B)(4|C)(7|F)(8|G))|((3|B)(4|C)(8|G)(7|F))|((3|B)(7|F)(4|C)(8|G))|((3|B)(7|F)(8|G)(4|C))|((3|B)(8|G)(4|C)(7|F))|((3|B)(8|G)(7|F)(4|C))|((4|C)(3|B)(7|F)(8|G))|((4|C)(3|B)(8|G)(7|F))|((4|C)(7|F)(3|B)(8|G))|((4|C)(7|F)(8|G)(3|B))|((4|C)(8|G)(3|B)(7|F))|((4|C)(8|G)(7|F)(3|B))|((7|F)(3|B)(4|C)(8|G))|((7|F)(3|B)(8|G)(4|C))|((7|F)(4|C)(3|B)(8|G))|((7|F)(4|C)(8|G)(3|B))|((7|F)(8|G)(3|B)(4|C))|((7|F)(8|G)(4|C)(3|B))|((8|G)(3|B)(4|C)(7|F))|((8|G)(3|B)(7|F)(4|C))|((8|G)(4|C)(3|B)(7|F))|((8|G)(4|C)(7|F)(3|B))|((8|G)(7|F)(3|B)(4|C))|((8|G)(7|F)(4|C)(3|B))|((3|B)(4|C))|((3|B)(4|C))|((3|B)(4|C))|((4|C)(3|B))|((4|C)(3|B))|((4|C)(3|B))|((3|B)(4|C))|((3|B)(4|C))|((4|C)(3|B))|((4|C)(3|B))|((3|B)(4|C))|((4|C)(3|B))|((3|B)(5|D)(7|F))|((3|B)(5|D)(7|F))|((3|B)(7|F)(5|D))|((3|B)(7|F)(5|D))|((3|B)(5|D)(7|F))|((3|B)(7|F)(5|D))|((5|D)(3|B)(7|F))|((5|D)(3|B)(7|F))|((5|D)(7|F)(3|B))|((5|D)(7|F)(3|B))|((5|D)(3|B)(7|F))|((5|D)(7|F)(3|B))|((7|F)(3|B)(5|D))|((7|F)(3|B)(5|D))|((7|F)(5|D)(3|B))|((7|F)(5|D)(3|B))|((7|F)(3|B)(5|D))|((7|F)(5|D)(3|B))|((3|B)(5|D)(7|F))|((3|B)(7|F)(5|D))|((5|D)(3|B)(7|F))|((5|D)(7|F)(3|B))|((7|F)(3|B)(5|D))|((7|F)(5|D)(3|B))|((4|C)(4|C)(6|E)(8|G))|((4|C)(4|C)(8|G)(6|E))|((4|C)(6|E)(4|C)(8|G))|((4|C)(6|E)(8|G)(4|C))|((4|C)(8|G)(4|C)(6|E))|((4|C)(8|G)(6|E)(4|C))|((6|E)(4|C)(4|C)(8|G))|((6|E)(4|C)(8|G)(4|C))|((6|E)(8|G)(4|C)(4|C))|((8|G)(4|C)(4|C)(6|E))|((8|G)(4|C)(6|E)(4|C))|((8|G)(6|E)(4|C)(4|C))|((4|C)(5|D)(6|E))|((4|C)(5|D)(6|E))|((4|C)(6|E)(5|D))|((4|C)(6|E)(5|D))|((4|C)(5|D)(6|E))|((4|C)(6|E)(5|D))|((5|D)(4|C)(6|E))|((5|D)(4|C)(6|E))|((5|D)(6|E)(4|C))|((5|D)(6|E)(4|C))|((5|D)(4|C)(6|E))|((5|D)(6|E)(4|C))|((6|E)(4|C)(5|D))|((6|E)(4|C)(5|D))|((6|E)(5|D)(4|C))|((6|E)(5|D)(4|C))|((6|E)(4|C)(5|D))|((6|E)(5|D)(4|C))|((4|C)(5|D)(6|E))|((4|C)(6|E)(5|D))|((5|D)(4|C)(6|E))|((5|D)(6|E)(4|C))|((6|E)(4|C)(5|D))|((6|E)(5|D)(4|C))|((5|D)(5|D)(6|E)(7|F))|((5|D)(5|D)(7|F)(6|E))|((5|D)(6|E)(5|D)(7|F))|((5|D)(6|E)(7|F)(5|D))|((5|D)(7|F)(5|D)(6|E))|((5|D)(7|F)(6|E)(5|D))|((6|E)(5|D)(5|D)(7|F))|((6|E)(5|D)(7|F)(5|D))|((6|E)(7|F)(5|D)(5|D))|((7|F)(5|D)(5|D)(6|E))|((7|F)(5|D)(6|E)(5|D))|((7|F)(6|E)(5|D)(5|D))|((6|E)(6|E)(9|H)(9|H))|((6|E)(9|H)(6|E)(9|H))|((6|E)(9|H)(9|H)(6|E))|((9|H)(6|E)(6|E)(9|H))|((9|H)(6|E)(9|H)(6|E))|((9|H)(9|H)(6|E)(6|E))|((6|E)(7|F)(8|G)(9|H))|((6|E)(7|F)(9|H)(8|G))|((6|E)(8|G)(7|F)(9|H))|((6|E)(8|G)(9|H)(7|F))|((6|E)(9|H)(7|F)(8|G))|((6|E)(9|H)(8|G)(7|F))|((7|F)(6|E)(8|G)(9|H))|((7|F)(6|E)(9|H)(8|G))|((7|F)(8|G)(6|E)(9|H))|((7|F)(8|G)(9|H)(6|E))|((7|F)(9|H)(6|E)(8|G))|((7|F)(9|H)(8|G)(6|E))|((8|G)(6|E)(7|F)(9|H))|((8|G)(6|E)(9|H)(7|F))|((8|G)(7|F)(6|E)(9|H))|((8|G)(7|F)(9|H)(6|E))|((8|G)(9|H)(6|E)(7|F))|((8|G)(9|H)(7|F)(6|E))|((9|H)(6|E)(7|F)(8|G))|((9|H)(6|E)(8|G)(7|F))|((9|H)(7|F)(6|E)(8|G))|((9|H)(7|F)(8|G)(6|E))|((9|H)(8|G)(6|E)(7|F))|((9|H)(8|G)(7|F)(6|E))|((6|E)(9|H))|((6|E)(9|H))|((6|E)(9|H))|((9|H)(6|E))|((9|H)(6|E))|((9|H)(6|E))|((6|E)(9|H))|((6|E)(9|H))|((9|H)(6|E))|((9|H)(6|E))|((6|E)(9|H))|((9|H)(6|E))|((7|F)(7|F)(8|G)(8|G))|((7|F)(8|G)(7|F)(8|G))|((7|F)(8|G)(8|G)(7|F))|((8|G)(7|F)(7|F)(8|G))|((8|G)(7|F)(8|G)(7|F))|((8|G)(8|G)(7|F)(7|F))|((7|F)(8|G))|((7|F)(8|G))|((7|F)(8|G))|((8|G)(7|F))|((8|G)(7|F))|((8|G)(7|F))|((7|F)(8|G))|((7|F)(8|G))|((8|G)(7|F))|((8|G)(7|F))|((7|F)(8|G))|((8|G)(7|F))}
